Neural Assistive Impulses: Synthesizing Exaggerated Motions for Physics-based Characters

Physics-based character animation has become a fundamental approach for synthesizing realistic, physically plausible motions. While current data-driven deep reinforcement learning (DRL) methods can synthesize complex skills, they struggle to reproduce exaggerated, stylized motions, such as instantaneous dashes or mid-air trajectory changes, which are required in animation but violate standard physical laws. The primary limitation stems from modeling the character as an underactuated floating-base system, in which internal joint torques and momentum conservation strictly govern motion. Direct attempts to enforce such motions via external wrenches often lead to training instability, as velocity discontinuities produce sparse, high-magnitude force spikes that prevent policy convergence. We propose Assistive Impulse Neural Control, a framework that reformulates external assistance in impulse space rather than force space to ensure numerical stability. We decompose the assistive signal into an analytic high-frequency component derived from Inverse Dynamics and a learned low-frequency residual correction, governed by a hybrid neural policy. We demonstrate that our method enables robust tracking of highly agile, dynamically infeasible maneuvers that were previously intractable for physics-based methods.

==> src/00-abstract.tex <==
\begin{abstract}
Physics-based character animation has become a fundamental approach for synthesizing realistic, physically plausible motions. While current data-driven deep reinforcement learning (DRL) methods can synthesize complex skills, they struggle to reproduce exaggerated, stylized motions, such as instantaneous dashes or mid-air trajectory changes, which are required in animation but violate standard physical laws. The primary limitation stems from modeling the character as an underactuated floating-base system, in which internal joint torques and momentum conservation strictly govern motion. Direct attempts to enforce such motions via external wrenches often lead to training instability, as velocity discontinuities produce sparse, high-magnitude force spikes that prevent policy convergence. We propose Assistive Impulse Neural Control, a framework that reformulates external assistance in impulse space rather than force space to ensure numerical stability. We decompose the assistive signal into an analytic high-frequency component derived from Inverse Dynamics and a learned low-frequency residual correction, governed by a hybrid neural policy. We demonstrate that our method enables robust tracking of highly agile, dynamically infeasible maneuvers that were previously intractable for physics-based methods.
\end{abstract}

==> src/10-figs.tex <==
\clearpage
\begin{figure*}[p] 
    \centering

    \includegraphics[width=0.99\linewidth]{img/tasks-small.pdf}
    \caption{Snapshots of the simulated humanoid characters trained using our NAI framework, showcasing exaggerated and stylized motion capabilities.}
    \label{fig:tasks}
    
    \vspace{0.5cm}
    \begin{minipage}[t]{0.99\linewidth} 
        \centering
        \includegraphics[trim=0 10cm 0 0, clip, width=\linewidth]{img/nai_native.pdf}
        \caption{Comparison of assistive intervention profiles of teaser motion. The \textbf{Native Assist} (red) exhibits continuous, high-frequency force fluctuations ("always-on"), indicating an over-reliance on external assistance to force kinematic compliance. In contrast, \textbf{Ours} (blue) demonstrates distinct \textbf{sparsity}: the assistive impulse drops to near-zero during physically consistent phases (e.g., $t=0.0s-0.3s$, $t=3.5s+$) and activates smoothly only when dynamic transients require momentum injection.}
        \label{fig:impulse_profile}
    \end{minipage}
    \hfill 
    \begin{minipage}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{img/spikes.png}
        \caption{Comparison between Force-space and Momentum-space control signals. We show the magnitude profiles of the assistive intervention for a simulated character performing the motion described in the teaser. While the instantaneous Assistive Force (solid lines) suffers from extreme magnitude spikes and dependency on simulation time-steps ($F \propto 1/\Delta t$), the integrated Assistive Impulse (blue dashed) provides a smooth, bounded, and frequency-invariant learning target for the neural policy.}
        \label{fig:spike}
    \end{minipage}
    
\end{figure*}
\clearpage

%
% \begin{figure}[hbt]
%     \centering
%     \includegraphics[trim=0 10cm 0 0, clip,width=\linewidth]{img/nai_native.pdf}
%     \caption{Comparison of assistive intervention profiles of teaser motion. The \textbf{Native Assist} (red) exhibits continuous, high-frequency force fluctuations ("always-on"), indicating an over-reliance on external assistance to force kinematic compliance. In contrast, \textbf{Ours} (blue) demonstrates distinct \textbf{sparsity}: the assistive impulse drops to near-zero during physically consistent phases (e.g., $t=0.0s-0.3s$, $t=3.5s+$) and activates smoothly only when dynamic transients require momentum injection.}
%     \label{fig:impulse_profile}
% \end{figure}

% \begin{figure}[hbt]
%     \centering
%     \includegraphics[width=0.99\linewidth]{img/spikes.png}
%     \caption{Comparison between Force-space and Momentum-space control signals. We show the magnitude profiles of the assistive intervention for a simulated character performing the motion described in the teaser. While the instantaneous Assistive Force (solid lines) suffers from extreme magnitude spikes and dependency on simulation time-steps ($F \propto 1/\Delta t$), the integrated Assistive Impulse (blue dashed) provides a smooth, bounded, and frequency-invariant learning target for the neural policy.}
%     \label{fig:spike}
% \end{figure}


% \begin{figure*}[hbt]
%     \centering
%     \includegraphics[width=0.99\linewidth]{img/tasks-small.pdf}
%     \caption{Snapshots of the simulated humanoid characters trained using our NAI framework, showcasing exaggerated and stylized motion capabilities.}
%     \label{fig:tasks}
% \end{figure*}




% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{img/delta_impulse.png}
%     \caption{Analysis of the Neural Residual mechanism of Teaser motion. Top: The Analytical Reference ($\mathbf{I}_{base}$) derived from offline RNEA provides a general momentum guide, but often underestimates the requirements due to simulation discrepancies (e.g., contact delays, friction errors). The Neural Residual Impulse ($\mathbf{I}_{total}$) shows how the policy augments the signal. Bottom: The difference $\Delta$ Impulse actively bridges this "dynamics gap," injecting additional momentum (positive peaks) or correcting timing mismatches to ensure robust tracking.}
%     \label{fig:residual_analysis}
% \end{figure}


==> src/macros.tex <==
\usepackage{color}
\usepackage{soul}
\usepackage{multirow}
\usepackage{rotating}
%\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{algorithmicx}
\usepackage{wrapfig}
%\hypersetup{draft}
\usepackage[normalem]{ulem}
\usepackage{booktabs}
%\usepackage{algorithm}
\usepackage{algpseudocode}  
\usepackage{esvect}
\usepackage{enumitem}
\definecolor{purple}{rgb}{0.65,0,0.65}
\definecolor{darkgreen}{rgb}{0.0, 0.5, 0.0}
\definecolor{darkred}{rgb}{0.5, 0.0, 0.0}
\definecolor{darkblue}{rgb}{0.0, 0.0, 0.5}
\definecolor{blue}{rgb}{0.0, 0.0, 1.0}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage[table]{xcolor}
\usepackage{tabularx}
\usepackage{adjustbox}
\definecolor{tableblue}{rgb}{240, 245, 255} 
%use this in running text
\newcommand{\on}{{\textit{on} }}
\newcommand{\off}{{\textit{off} }}

%use this in image captions
\newcommand{\ON}{{\textup{on} }}
\newcommand{\OFF}{{\textup{off} }}
\newcommand{\OFFCapital}{{\textup{Off} }}

\newcommand{\todo}[1]{{\bf \color{red}[todo: #1]}}
%\newcommand{\changed}[1]{{\color{blue}#1}}
\newcommand{\changed}[1]{{#1}}
%\newcommand{\erase}[1]{\st{#1}}
\newcommand{\erase}[1]{}
\newcommand{\rep}[2]{{\bf \color{cyan}[replace: #1 {\it with} #2]}}

\newcommand{\BB}[1]{{\textbf{ \color{blue}[BB: #1]}}}
\newcommand{\bb}[1]{{\textbf{ \color{blue}[BB: #1]}}}

\newcommand{\zw}[1]{{\textbf{ \color{cyan}[ZW: #1]}}}
\newcommand{\ZW}[1]{{\textbf{ \color{cyan}[ZW: #1]}}}


\newcommand{\QA}[1]{{\textbf{ \color{orange}[QA: #1]}}}
\newcommand{\qa}[1]{{\textbf{ \color{orange}[QA: #1]}}}

\newcommand{\sd}[1]{{\bf \color{darkgreen}[SD: #1]}}
\newcommand{\SD}[1]{{\bf \color{darkgreen}[SD: #1]}}

\newcommand{\hk}[1]{{\bf \color{purple}[HK: #1]}}
\newcommand{\HK}[1]{{\bf \color{purple}[HK: #1]}}

\newcommand{\NC}[1]{{\bf \color{blue}[NC: #1]}}
\newcommand{\nc}[1]{{\bf \color{blue}[NC: #1]}}

\newcommand{\EY}[1]{{\bf \color{turquoise}[EY: #1]}}
\newcommand{\ey}[1]{{\bf \color{turquoise}[EY: #1]}}

\newcommand{\AS}[1]{{\bf \color{blue}[AS: #1]}}
\newcommand{\as}[1]{{\bf \color{blue}[AS: #1]}}

\newcommand{\xw}[1]{{\bf \color{purple}[XW: #1]}}
\newcommand{\XW}[1]{{\bf \color{purple}[XW: #1]}}


\newcommand{\meta}[1]{{\color{blue}[meta: #1]}}
\newcommand{\hide}[1]{{}}
\newcommand{\ch}[1]{{#1}}
\newcommand{\eg}{{\textit{e.g., }}}
\newcommand{\ie}{{\textit{i.e., }}}

% Gundy
\definecolor{darkblue}{rgb}{0.0, 0.2, 0.5}
\newcommand{\gon}{\color{darkblue}}
\newcommand{\goff}{\color{black}}
\newcommand{\todogundy}[1]{\marginpar{\color{darkblue}\small\textbf{Gundy}}{\color{darkblue}#1}\par}
\newcommand{\warn}{\color{red}}
\newcommand{\gundyon}{\color{darkblue}}
\newcommand{\gundyoff}{\color{black}}

%Adrien

\newcommand{\AP}[1]{{\textbf{ \color{blue}[AP: #1]}}}
\newcommand{\ap}[1]{{\textbf{ \color{blue}[AP: #1]}}}

\newcommand{\mbf}[1]{\mathbf{#1}}
\renewcommand{\vec}[1]{\mathbf{#1}}
%\newcommand{\norm}[1]{\lVert #1 \rVert}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\abs}[1]{\lvert #1 \rvert}

\newcommand{\argmax}[1]{\underset{#1}{\operatorname{arg}\,\operatorname{max}}\;}
\newcommand{\argmin}[1]{\underset{#1}{\operatorname{arg}\,\operatorname{min}}\;}

%% REVISION MACROS
%\newcommand{\rev}[2]{{\bf \color{blue}\textsuperscript{#1}#2}}
%\newcommand{\revimage}[1]{\fcolorbox{blue}{blue}{#1}}
%\newcommand{\revremove}[1]{{\bf \color{red}[\st{#1}]}}




%% REVISION 2 MACROS
%\newcommand{\revtwo}[2]{{\bf \color{darkgreen}\textsuperscript{#1}#2}}
%\newcommand{\revimagetwo}[1]{\fcolorbox{darkgreen}{darkgreen}{#1}}

%% REVISION 3 MACROS
%\newcommand{\revthree}[2]{{\bf \color{red}\textsuperscript{#1}#2}}

\newcommand{\rev}[2]{{#2}}
\newcommand{\revimage}[1]{{#1}}
\newcommand{\revtwo}[2]{{#2}}
\newcommand{\revimagetwo}[1]{{#1}}
\newcommand{\revthree}[2]{{#2}}

%\newcommand{\qa}[2]{\marginpar{\color{blue}\textbf{#1}}{\color{red}#2}}
\usepackage{marginnote}
%\newcommand{\qa}[2]{\protect\marginnote{\color{blue}\textbf{#1}}{\color{red}#2}}


